Fully upgraded $\beta$-NMR setup at ISOLDE for high-precision high-field studies

$\beta$-NMR is an advancing technique that enables measurements relevant to various fields of research, ranging from physics to chemistry and biology. Among the recent achievements of the $\beta$-NMR setup located at the ISOLDE facility at CERN is the determination of the magnetic moment of a shortlived nucleus with a part-per-million accuracy. Presented here are major upgrades and extensions of that $\beta$-NMR setup. The most important advancement is the installation of a 4.7 T superconducting solenoidal magnet, leading to sub-ppm spatial homogeneity and temporal stability of the magnetic field. A detector array optimised for such magnetic field has also been implemented and a more powerful, time-resolved, fully-digital data acquisition system has been deployed. To commission the upgraded beamline, $\beta$-NMR resonances of short-lived 26Na were recorded in solid and liquid samples. These showed 3-fold narrower linewidths and 15-fold higher resolving power than using the previous setup. Hence, the improvements achieved here permit more accurate bio-$\beta$-NMR studies, investigating, e.g., the interaction of metal ions with biomolecules, such as DNA. They also pave the way for the first studies of the distribution of the magnetisation inside short-lived nuclei.

==> Sections/01_00-Introduction.tex <==

\section{Introduction}

% Introduction bNMR
Nuclear magnetic resonance (NMR) is a powerful spectroscopic technique used in physics, chemistry and biology \cite{Mazzola03}.
It relies on the interaction of nuclear spins with static and periodic magnetic fields. NMR can yield information on the probed nuclei and their environment \cite{Abragam1989,Mazzola03} through their Larmor precession frequency and relaxation time that reflects the speed at which they return to thermal equilibrium.
The strength of the registered signal depends on the spin polarisation (or orientation), which depends on the population difference between different spin orientations \cite{Stone1986}.
A high polarisation is thus beneficial and different techniques are used to achieve it in stable nuclei, e.g.\ dynamic nuclear polarisation, parahydrogen-induced polarisation or optical pumping \cite{Halse2016}.
The latter refers to laser light `pumping' selected energy levels of an atom and has been also extensively used for radiation-detected NMR on short-lived isotopes at ISOLDE. 
Using circularly polarised laser light (\sigmap or \sigmam) allows to excite selectively transitions between magnetic sub-states $m_F$ of hyperfine states $F$.
This results in the sub-state $m_F=\pm F$ obtaining an increased population and in return the atomic spin $F$ being polarised.
Through the hyperfine interaction, this also leads to a polarisation of the nuclear spin $I$. % the electron spin $J$.

\bNMR is a technique that benefits not only from hyperpolarisation of the nuclear spin like conventional NMR, but goes one step further in the increase of sensitivity. 
Due to the parity violation of the weak force, a nuclear spin polarisation also takes effect on radioactive isotopes in the form of an anisotropy in the \btext decay \cite{Wu1957}.
\bNMR utilises the change of this effect over time or under rf excitation as efficient means of detecting resonances \cite{Kowalska2008}.


The main application of \bNMR so far has been in nuclear physics, where it has allowed to investigate spins %$I$
\cite{Kowalska2008}, magnetic dipole moments
%$\mu_I$ 
\cite, and electric quadrupole moments
%$Q$ 
\cite{Keim2000, Yordanov2019} of unstable nuclei in solid hosts.
A recent achievement of the technique has been the determination of the magnetic moment $\mu_I$ of \textsuperscript{26}Na with an unprecedented parts-per-million accuracy \cite{Harding2020MagneticBiology}.
For this, a beam of \textsuperscript{26}Na was implanted in a liquid sample.
The molecular tumbling in the sample averaged out anisotropic contributions \cite{Abragam1989}, resulting in an NMR resonance two orders of magnitude narrower than in a conventional solid-state sample \cite{Croese2021}.
Such precise magnetic moments can be combined with measurements of the hyperfine structure to determine the hyperfine anomaly and yield information on the distribution of nuclear magnetisation and the neutrons in the nucleus \cite{Bissell2023}.
% Further applications and transition to biochemistry
Moreover, liquid-state \bNMR starts being applied to other research fields, including material sciences \cite{MacFarlane2015, Ruiz2015}, and chemistry \cite{Gottberg2014, Szunyogh2018}.
A promising, novel application lies in biochemistry, which requires the measurement of small chemical shifts \cite{Jancso2017} to, e.g., investigate the interaction of DNA structures with alkali metals, such as Na or K \cite{Karg2020}.
These DNA studies are barely feasible in conventional Na or K NMR because of the low sensitivity and peak broadening due to the quadrupolari interaction of spins $I>1/2$ of the used stable 23Na and 39,41K \cite{Karg2022} with the electric field gradients or electric field fluctuations in the liquid hosts.
This issue can be overcome by \bNMR which does not only enable studies with more $I=1/2$ nuclei in form of short-lived radioactive isotopes, but, more importantly, offers significantly higher sensitivity \cite{Gottberg2014}.

% explanation of VITO and its approach
The \bNMR setup described in this manuscript is already up to ten orders of magnitude more sensitive than conventional NMR \cite{Kowalska2017}, thus allowing, e.g., measurements with significantly fewer nuclei \cite{Gottberg2014}.
Two key features primarily contribute to this boosted sensitivity:
First, a great degree of nuclear polarisation is achieved through optical pumping with circularly polarised laser light, proportionally enhancing the signal amplitude \cite{Stone1986}.
Second, highly efficient detectors record the \btext particles emitted by the radioactive nuclei and in return their asymmetry, giving a potent means of recording NMR spectra \cite{Kowalska2017}.
% bNMR not ready yet - need to improve the resolution
While the sensitivity of \bNMR is predestined for biochemical applications, the resolution of the already improved setup \cite{Croese2021} needs to be enhanced for the upcoming biochemistry studies; investigating the interaction of alkali metals with DNA structures \cite{Karg2020, Karg2022}.

This contribution gives an overview on the major upgrades of the \bNMR beamline at ISOLDE to improve further its resolution. 
The improvements include a 4.7~T superconducting magnet, a new \btext $\beta$-detector array and a versatile, time-resolved digital data acquisition system.
To commission the setup, \bNMR resonances of \textsuperscript{26}Na in a crystal and in ionic liquids were recorder and compared to the previous beamline \cite{Harding2020MagneticBiology,Croese2021}.


==> Sections/02_01-General_upgrades.tex <==



==> Sections/05_00-MagneticMoment.tex <==
\section{New magnetic moment 26Na}

include Andrejs for shielding for 23Na as new reference

stable 23Na in H2O in good agreement with literature, see FID\_analysis\_Mark.xlsx. But: frequencies for 2H and Na have not been corrected for susceptibility or shielding?
where did Mark's literature value come from?

==> Sections/07_00-Contributions.tex <==
\section{Contributions}
\textbf{MORE elements should/could be added.}
MK obtained funding for hardware and part of manpower.
NA, JC, SW, MJ designed the sample carriage, detector box, and back chamber.
SW performed beam optics calculations that influenced the position of the beam focusing elements and of the magnet.
SW, BK, NA coordinated the magnet installation at ISOLDE.
SW designed and simulated in the \btext detectors in GEANT4.
MM and the MMF workshop manufactured the detectors.
MM and SW characterised and assembled the detectors.
MCh performed GEANT4 simulations to determine the \textbeta-decay asymmetry for \textsuperscript{26}Na in presence of magnetic fields.
HB, JC and MJ programmed the DAQ.
MB made the RF coils for \bNMR and the \textsuperscript{2}H NMR probe with electronics for \textsuperscript{2}H pulsed-NMR.
KDK and BK were preparing the liquid samples.
LVR, MLB prepared the lasers.
MJ performed the data analysis.
MJ and MK wrote the manuscript.
All co-authors participated in the preparations for and online beamtimes.
All co-authors made comments to the manuscript.

==> Sections/Old_order/02_00-Methods.tex <==
\section{Methods}
\label{section:Setup}
% Ziel formulieren statt "dedicated" zu nutzen. Ziel benennen und sagen, dass beamline dafür verwendet wird

The experimental setup described in this manuscript is designed to perform \bNMR experiments on beams of unstable nuclei.
For this purpose, the beam provided by the ISOLDE facility at CERN \cite{Gottberg2016, Borge2016, Borge2017, Catherall2017} needs to be polarised.
Circularly polarised laser light (\sigmam/\sigmap) excites the magnetic sub-states $m_F$ of a selected hyperfine state $F$ in a weak magnetic field, resulting in one of the sub-states obtaining an increased population.
This process is called optical pumping.
The beam is set into resonance with the laser by changing its velocity with an offset potential, which is referred to as Doppler tuning \cite{Gins2019}.
By optical pumping, the atomic spin $F$ is polarised, which in turn also polarises the nuclear spin $I$ through the hyperfine interaction.
Finally, the polarised beam enters a strong magnetic field and is then implanted into a sample.
The polarisation is visible as an asymmetry in the emission of \textbeta~particles from the decaying nuclei \cite{Wu1957}, which is measured with two detectors, located around the sample along and against the field direction.
To record a hyperfine structure splitting (HFS), the \textbeta~asymmetry is measured as a function of the perceived laser frequency by scanning the Doppler tuning voltage.
For an NMR measurement, the isotope beam is brought into resonance with light at the perceived laser frequency yielding the highest \textbeta~decay asymmetry, and a RF field is applied around the sample.
The \textbeta~asymmetry is then acquired as a function of the RF frequency to record a NMR resonance.

This section describes in more detail the most important upgrades that have recently been implemented at the \bNMR beamline,  with the setup and its components in its current state depicted in Figure \ref{fig:beamline} including the wide-bore superconducting magnet and additional beam focusing elements.

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{Figures/Beamline_overview.pdf}
    \caption{Overview on the components of the upgraded \bNMR beamline: (1) quadrupole doublet, (2) bender, (3) quadrupole triplet, (4) Doppler tuning electrode, (5) charge exchange cell, (6) optical pumping section, (7) detector chamber, (8) superconducting magnet, (9) retractable sample carriage.}
    \label{fig:beamline}
\end{figure*}

\input{Sections/02_01-Beamline_Upgrade}

\input{Sections/02_02-Detector_design}

\input{Sections/02_03-DAQ_methods}

\input{Sections/02_04-Data_methods}

==> Sections/Old_order/02_01-Beamline_Upgrade.tex <==
\subsection{Beamline upgrades}

One drawback of the previous \bNMR setup at ISOLDE \cite{Croese2021} is a relatively low homogeneity of the electromagnet's 1.2~T field.
To tackle this issue, a superconducting magnet (Bruker 47/16) with a magnetic field of 4.7~T has been implemented, cf. (8) in Figure \ref{fig:beamline}.
The magnet has a bore with a diameter of 160~mm that accommodates the last beamline section with the sample in its centre. 
Further components located inside the magnet include the RF coil and the rear detector, both of which are fixed on an aluminium breadboard, \textbf{referred to as the `sample carriage' (9)}.
The carriage rests on a rail system, allowing it to be easily retracted from the centre of the magnet, e.g. for a sample change\textbf{, with numerous fixing points available for a modular an adaptable design}. 
It also hosts a removable Faraday cup is installed along with a D\textsubscript{2}O NMR probe. 
%This probe is located at a distance of XX~mm from the sample to perform NMR with a reference isotope (here \textsuperscript{2}H) and determine the exact magnetic field $B$.
When the sample carriage is inserted into the magnet, conical pins align it with the rest of the beamline, thus ensuring a fast and highly reproducible positioning of all components with reference to the beam axis.

%\begin{figure}
%    \centering
%    \includegraphics[width=\columnwidth]{Figures/BackFlangeS%uport.png}
%    \caption{Sample carriage with (a) sample holder, (b) Faraday cup, (c) NMR probe and (d) rear detector. %(\textbf{deuterium probe and rear detector are not in %drawing}).}
%    \label{fig:SampleCarriage}
%\end{figure}




==> Sections/Old_order/03_00-Results_Discussion.tex <==
\section{Results and discussion}
\label{section:Results}

%This part of the manuscript evaluates the upgrades performed at the \bNMR beamline and recommissions it by acquiring online data and comparing it to the outcome of the previous setup.


% All three graphs are based on the same measurement with 2~s acquisition time per data point, but the depicted \btext asymmetries are calculated for different observation windows of 0.4~s to 0.8~s, 1.6~s to 2~s and the default 0~s to 2~s.
% The data sets indicate the maximum asymmetry at a Doppler voltage of -1.12~V. 
% Their amplitude, however, differs depending on the observed time window.
% baseline -1.5 %; 0.4:0.8s -7.9 %; 1.6:2s -6.6 %; 0:2s -7.4 %
% amplitudes: beginning 6.4 %, ending 5.1 %, total 5.9 %
% Computing the \btext asymmetry based on the entire measurement duration of 2~s per data point leads to an amplitude of 5.9~\%.
% An amplitude loss of 0.8~\% is registered for the observation window of 1.6~s to 2~s while an amplitude gain of 0.5~\% is experienced in case of the 0.4~s to 0.8~s observation window. 
% The implantation of spin-polarised atoms stops at 0.5~s after the trigger signal.
% From this point on, the recorded \textbeta\ particles are all emitted by the atoms that are remaining in the sample.
% Thus, the difference in the \textbeta\ asymmetry amplitude for the respective observation windows is caused by the ratio of nuclei whose spin polarisation has already relaxed by that time, which explains why the observation window from 0.4~s to 0.8~s has the highest amplitude.
% This illustrates how the spectrum is influenced by the observation window and how a carefully tuned time window can benefit the signal to noise ratio, when the relaxation time and the uncertainty from the number of \textbeta\ particles within that observation window are taken into account.
% The new DAQ recording time-resolved data hence enables the user to select the observation window that maximises the signal amplitude. (maybe for summary)

\input{Sections/03_01-Beamline_results}
\input{Sections/03_02-Detector_results}
\input{Sections/03_03-DAQ_results}
\input{Sections/03_04-Data_results}

==> Sections/Old_order/03_01-Beamline_results.tex <==
\subsection{Beamline upgrades}

%The implementation of the superconducting Bruker 47/16 MRI magnet is the most substantial upgrade to the beamline.
%Its magnetic field of 4.7~T represents a fourfold increase compared to the previously used electromagnet, which will benefit the frequency resolution of the NMR measurements. % reference...
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{Figures/mapa.png}
    \caption{Homogeneity of the $B$-field in the centre of the superconducting magnet. \textbf{this rather unpretty figure will be replaced when Mik sends the missing data}}
    \label{fig:MagFieldMap}
\end{figure}
The magnetic field of 4.7~T represents a fourfold increase compared to the previously used electromagnet \cite{Croese2021}.
As the homogeneity of its magnetic field was optimised at the magnet's final location, it reaches sub-ppm values across the region of the sample and the reference NMR probe, see Figure \ref{fig:MagFieldMap}. % Refer to plot of the field measured by Mik. Ideally, show field around the sample in the centre and the D2O probe
Additionally, the magnet is characterised by a high temporal stability of the magnetic field with a drift below 0.06~ppm/h.

\cite{Croese2021}. %, which showed fluctuations of $\pm0.6$~ppm even with an active field stabilisation \cite{Croese2021}.

% The magnet offers an active shielding, thus diminishing stray fields.
With the magnet being a solenoid, its $B$-field is oriented along the beam axis rather than perpendicular to the beam. 
% A rotation of the spins into the magnetic field is hence not required, as it was the case of the previously used electromagnet \cite{Croese2021}, and resulting polarisation losses are prevented.

These changes largely contribute to improving the signal to noise ratios of the detected \textbeta\ asymmetries.
In addition, the sample carriage improves the reproducibility of the components inside the superconducting magnet
Thus, it diminishes the uncertainty of the difference in the magnetic field between the sample and the reference NMR probe compared to the previous setup \cite{Harding2020MagneticBiology}.


==> Sections/Old_order/03_02-Detector_results.tex <==
\subsection{Detectors}
This section describes the final design and evaluation of the new detectors.

Both detectors use thin plastic scintillators (material?) and silicon photomultipliers (model?).
The latter are not influenced by the strong magnetic field of the superconducting magnet and can hence even be located close to the sample, without the need of using light guides.
The front detector comprises a XX mm large aperture to let the atom beam pass through its centre towards the sample.
The gyro radii and the trajectory of the emitted \textbeta\ particles, have led to a design of the front detector array in the form of a funnel, see Figure XXX (CAD drawing to be added here).

To leave enough space for an aperture large enough to let the entire atom beam pass through without interfering with the detectors, the front detector is located outside the solenoid in a dedicated vacuum chamber, referred to as the detector box, circa 1~m away from the sample.

The rear detector is a 5-mm thick square scintillator with silicon photomultipliers. It is located inside the solenoid at a distance of XXX~mm to the sample. 
Due to a different geometry of the detectors, there will be an instrumental \textbeta\ decay asymmetry even in absence of spin polarisation, which is due to a different number of beta particles detected in the front and back detector. The beta-decay asymmetry due to change in spin polarisation (e.g. due to RF excitation) can be determined after subtracting the instrumental asymmetry.
